Computing Education in the Era of Generative AI

The computing education community has a rich history of pedagogical innovation designed to support students in introductory courses, and to support teachers in facilitating student learning. Very recent advances in artificial intelligence have resulted in code generation models that can produce source code from natural language problem descriptions -- with impressive accuracy in many cases. The wide availability of these models and their ease of use has raised concerns about potential impacts on many aspects of society, including the future of computing education. In this paper, we discuss the challenges and opportunities such models present to computing educators, with a focus on introductory programming classrooms. We summarize the results of two recent articles, the first evaluating the performance of code generation models on typical introductory-level programming problems, and the second exploring the quality and novelty of learning resources generated by these models. We consider likely impacts of such models upon pedagogical practice in the context of the most recent advances at the time of writing.

==> summarytables.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{p{.025\textwidth}|p{.3\textwidth} |p{.25\textwidth} |p{.02\textwidth} |p{.3\textwidth}} % {l|l|l}
        \hline
2.1.1 & We observed that some of the Codex answers contained trivial formatting errors. &  & 3.2 & LLm better programming error messages \\
2.1.1 & problems that disallowed the use of certain language features &  & 3.1 & LLM problem generation (priming) \\
2.1.2 & Codex struggled on cases where no valid values were provided as input &  & 3.1 & LLM problem generation (priming) \\
2.2.1 & academic misconduct & invigilate &  &  \\
2.2.2 & diverse range of views on the acceptability of code reuse & early concepts &  &  \\
2.2.3 & code reuse and licensing & early concepts \& practice &  &  \\
2.3.1 & over-reliance & early detect so as to teach &  &  \\
2.3.1 & over-reliance & early testing / requirements definition &  &  \\
2.4.1 & too advanced or complex for beginners & ? & 3.1 & LLM explanations (!) \\
2.4.3 & poor security practices & early security &  &  \\
   \end{tabular}
    \caption{Table direct from the text}
    \label{tab:table_textish}
\end{table*}

\textbf{Table~\ref{tab:table_shortlong} mixes wrong things together. Have a look and think whether any of the items are useful to us.}

\newlist{compactlist}{itemize}{1}
%% \setlist[testlist,1]{resume,leftmargin=*,label=(\arabic*)}
\setlist[compactlist,1]{leftmargin=*,label=\arabic*}


\begin{table*}[t]
    \centering
    \begin{tabular}{p{.13\textwidth}|p{.5\textwidth} |p{.3\textwidth}} % {l|l|l}
        \hline
            \textbf{Challenge} & \textbf{Short-term} & \textbf{Long-term}  \\
        \hline

overreliance & early-detection to help students learn meta-cognitive skills before they become overwhelmed &

%% \item \makecell[l]{teach unit testing early \\ teach theory early, \\ such as 'weakest precondition' }\\
\begin{compactlist} 
\item[*] early: unit testing
\item[*] early: theory e.g. 'weakest precondition' 
\item[*] early: code reviews
\item[*] emphasize \emph{reading} skills over \emph{writing} skills
\end{compactlist} \\
\hline
        
%% \multicolumn{3}{l}{Academic misconduct: philosophy}\\ 
\multirow{4}{.12\textwidth}{academic misconduct: philosophy} & revisit our student learning outcomes & get involved in CS2023 ACM Curriculum \\
 & {\raggedright revisit existing accepted incremental-completion tools} & continue \\
 & early discussion of attribution & continue \\
 & early discussion of licensing & continue \\
%% \multicolumn{3}{l}{Academic misconduct: act}\\ 
\hline
\multirow{4}{.12\textwidth}{academic misconduct: act} & increase invigilated assessments & continue \\
 & Since codex is bad about "disallow" i.e. restrictions, use two types: 
 \begin{compactlist} 
 \item[] programming language (no functions!) 
 \item[] domain (max 3 trucks for deliveries)
 \end{compactlist} & no - GPT will be able to handle restrictions \\
 & publish all student code (blockchain?) (de-identified?) so that better tools in the future can find as-of-yet-undetected cheating & continue with ePortfolios \\
 \hline
%% \multicolumn{3}{l}{clarify distinctions}\\
 clarify distinctions & distinguish issues of LEARNING from those of PROFESSIONAL CONDUCT & continue \\
 &  &  \\
expectations & expect it to work about half of the time & expect it to work all of the time \\
 & since current LLMS produce "brittle" and "prompt"-dependent code, much of the 'wrong code' is easy to rule out & all generated code will run, so it will be more difficult to find 'hidden' limits that aren't in the prompt explicitly \\
 &  &  \\

 shaping output & unreliable, constraints in prompts not reliably handled & ability to shape output, e.g.: \\
 &  & "use Object Oriented approach" \\
 &  & "use Design Patterns" \\
 &  & "use best practices for security aspects" \\
 &  & "Optimize X over Y" (e.g. memory over speed) \\
 &  & "include code coverage tests" \\
 &  &  \\
 &  &  \\

 integration & N/A ? & "use COMPANYX-CRM as backend" \\
 &  & "use API-XYZ" \\
 &  & "use identity management X v2.3" \\
 &  &  \\
watermarks & N/A & reliable and accepted code signatures \\
 &  & Code Labels: ?? \\
 &  & Serving size: 64gb 8-core linux \\
 %% & & \parbox{\textwidth}{Contents: \begin{itemize}
 & & Contents: \begin{itemize}
 \item GNU abc v3.8 
 \item jupyter\_core v5.1.2 
 \item Bubba\'s amazingness v68
 \end{itemize} \\
 
   \end{tabular}
    \caption{Challenges and their short-term and long-term implications}
    \label{tab:table_shortlong}
\end{table*}
